Understanding the Energy Impact of Software Refactoring: A Workload-Aware Study of Controlled Examples and Real-World Commits

Refactoring improves software maintainability while preserving functional behavior, yet behavior preservation does not imply energy neutrality. Existing studies primarily examine isolated refactorings under fixed or simple workloads, leaving the effects of workload variation, real-world refactoring practices, explanatory factors, and energy regression identification insufficiently understood. We present the first large-scale empirical study of the energy impact of refactoring across two complementary Java benchmarks: a Micro-benchmark, comprising 68 refactoring types evaluated under diverse workloads, and a Practical-benchmark, containing 481 real-world refactoring commits from 430 GitHub projects. Using repeated paired energy measurements, we analyze workload sensitivity, refactoring patterns, explanatory factors, and the effectiveness of metric- and LLM-based regression identification. In the Micro-benchmark, 199 of 384 refactoring-workload pairs (51.8%) exhibit statistically significant energy differences, and 45.3% of refactoring instances change energy-impact classification across workloads. In the Practical-benchmark, only 36 commits (7.5%) show significant energy changes, although two-thirds differ by at least 10%. Refactoring type alone is insufficient to predict energy outcomes, while certain recurring refactoring combinations are associated with energy reductions. Changes in execution time consistently explain energy variation in the controlled benchmark but correlate weakly with energy changes in real-world commits. Our findings highlight the need for workload-diverse evaluation of the energy impact of refactoring; neither existing metric-based approaches nor LLM-based predictors can reliably identify refactoring-induced energy regressions, motivating the development of more accurate techniques for predicting the energy impact of refactoring.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

\subsection{Program Energy Consumption}
Refactoring engine



==> sections/experiments_old.tex <==
\section{Experiments}
\label{sec:experimental_design}

To study the impact of refactoring on energy consumption (RQ1) and identify which types of refactoring are more likely to influence energy consumption (RQ2), we analyze the energy measurements collected for both \microbenchmark{} and \practicalbenchmark{}. To answer RQ3, we evaluated energy-regression identification approaches by comparing metric-based learning models and LLM-based predictor under the same labeling and evaluation protocol.

\subsection{Experimental Setup}
\label{subsec:experimental_setup}
We use JoularJX~\cite{noureddine-ie-2022} to measure the energy consumption of Java programs. JoularJX is a Java-based software power-monitoring tool that can report energy consumption during program execution. It supports multiple operating systems and builds on platform-specific power interfaces, such as RAPL on Linux and \texttt{powermetrics} on macOS.

All measurements are conducted on a dedicated Mac mini server running macOS with an Apple M4 Pro processor and 24 GB of memory. During measurement, we keep the execution environment stable by avoiding unrelated workloads and disabling non-essential background activity when possible. Each benchmark item is measured on the same machine, with the same Java version, build configuration, and measurement tool setup for both the before and after versions.

Energy measurement is sensitive to runtime variability caused by JVM execution, operating-system scheduling, background activity, and thermal effects. To reduce these sources of noise, we use repeated measurements for every benchmark item. Before collecting measurements, we perform a short warm-up run. Between consecutive measurements, we insert a cool-down interval to reduce the influence of thermal accumulation. We also randomize the measurement order of the before and after versions within each pair to avoid systematic bias from always measuring one version first. For every run, we record raw energy consumption and execution-time data for subsequent statistical analysis.


\subsection{RQ1 and RQ2}
\label{subsec:experiment_rq1_rq2}

To answer RQ1 and RQ2, we test whether refactoring leads to a statistically significant change in energy consumption between the original (parent) version and the refactored version for both \microbenchmark{} and \practicalbenchmark{}. For each subject, we collect paired energy measurements before and after refactoring under the same workload, yielding two paired samples per subject. We apply the paired Wilcoxon signed-rank test~\cite{rosner2006wilcoxon} to determine whether the mean of the paired differences is non-zero. We choose Wilcoxon because (i) our measurements are paired by construction and (ii) energy measurements may not follow a normal distribution, making a non-parametric paired test more robust. We report statistical significance at a conventional level (e.g., $\alpha = 0.05$) and complement $p$-values with effect sizes. In addition to statistical significance, we quantify the magnitude of the energy change using Cliff's delta~\cite{macbeth2011cliff}. Cliff's delta is a non-parametric effect size that measures the degree of stochastic dominance between the after and before distributions. Reporting effect size is important because a statistically significant result may still correspond to a negligible practical change when the measurement variance is low.

\paragraph{Correlation analysis for \microbenchmark{}.}
Beyond comparing energy before vs.\ after refactoring, we further explore whether energy changes correlate with simple code metrics in \microbenchmark{}. Because the programs in \microbenchmark{} are small and self-contained, we do not compute the full commit-level metric families in Table~\ref{tab:extracted_metrics}. Instead, for each refactoring example, we compute a small set of lightweight metrics for the program before and after refactoring, including: (1) total number of changed lines, (2) cyclomatic complexity, (3) cognitive complexity, and (4) representative CK metrics such as coupling between objects (CBO). We then compute the Pearson correlation coefficient~\cite{sedgwick2012pearson} between the change in energy and the change in each metric. Pearson correlation is used here as a simple first-pass analysis to characterize the linear association between energy change and metric change in the controlled setting of \microbenchmark{}.



All statistical analyzes for RQ1 (Wilcoxon test, Cliff's delta, and Pearson correlation) are implemented using SciPy~\cite{scipylink}.


\paragraph{Correlation study for refactoring co-occurrence patterns.}
To examine whether certain refactoring operations tend to appear together and are associated with refactoring-induced energy changes, we also conduct a correlation study over refactoring co-occurrence patterns. For each refactoring commit where RefactoringMiner succeeds to detect refactoring types, we treat each detected refactoring type as a binary feature indicating its \emph{presence} (i.e., the corresponding RefactoringMiner counter is greater than zero). We then enumerate all refactoring pairs and triples present in each commit (using $k$-combinations over the set of present refactoring types), and keep only patterns whose support is at least a user-specified threshold (e.g., $\ge 10$ commits) to reduce noise from extremely rare patterns.

\paragraph{Statistical test and effect sizes.}
For each candidate pattern $S$ and each outcome $Y$ (significant \& energy increase, or significant \& energy decrease), we build a $2{\times}2$ contingency table where $a$ is the number of commits with $S$ present and $Y{=}1$, $b$ is the number with $S$ present and $Y{=}0$, $c$ is the number with $S$ absent and $Y{=}1$, and $d$ is the number with $S$ absent and $Y{=}0$. We quantify association using (i) \emph{confidence} $P(Y{=}1\mid S)$ and \emph{lift} (confidence divided by the outcome base rate), (ii) \emph{odds ratio} (with a $0.5$ correction when any cell is zero), and (iii) the $\phi$ coefficient as a correlation-like effect size. We assess statistical significance using Fisher's exact test (two-sided)~\cite{fay2010two} and apply Benjamini--Hochberg false discovery rate (BH-FDR) correction~\cite{thissen2002quick} across all tested patterns for each outcome and pattern size ($k{=}2$ or $k{=}3$), reporting the adjusted $q$-values.
 


\subsection{RQ3}
\label{subsec:experiment_rq3}
\paragraph{Accounting for JVM JIT effects.}
Previous work shows that JVM execution characteristics can be affected by JIT compilation, especially for frequently executed code paths~\cite{10.1145/3485136,jia2023detecting}. Since our \microbenchmark{} programs are executed many times, JIT optimization can influence the measured energy change ratio. To examine this factor explicitly, we measure the energy consumption for each refactoring example under two execution modes: (i) default JVM execution (JIT enabled) and (ii) interpreter-only execution by setting \texttt{-Xint}~\cite{jitswitch} (JIT disabled). For each mode, we execute the program for a fixed number of iterations (1{,}000{,}000 iterations in our experiments) to obtain stable energy measurements, and we compute the energy change ratio between the refactored and original versions. We then compute Pearson correlation between (a) energy before vs.\ after refactoring and (b) the derived energy change ratio, under both JIT-enabled and JIT-disabled settings, to assess whether conclusions are sensitive to JIT behavior.


\subsection{RQ4}
\label{subsec:experiment_rq4}

To answer RQ3, we evaluated two classes of approaches for predicting whether a refactoring commit induces an energy regression: (i) metric-based machine learning models trained on extracted commit features, and (ii) an LLM-based predictor prompted with the same information. Because no existing tool is specifically designed for refactoring-induced energy regression, we adapt established commit-level regression prediction practices from previous work on performance-bug prediction using code metrics~\cite{10.1145/3643991.3644920}.

\paragraph{Ground-truth labels.}
For each refactoring commit in \practicalbenchmark{}, we obtain the binary label \textsc{Reg} vs.\ \textsc{NotReg} based on the paired before/after energy measurements and the statistical procedure described in Section~\ref{subsec:experiment_rq1_rq2}. This label serves as the ground truth for both metric-based and LLM-based predictions.

\subsubsection{Metric-based prediction models} We use the extracted metric families listed in Table~\ref{tab:extracted_metrics} (static code metrics, code change metrics, test metrics, refactoring metrics, and semantic metrics) as input for the model. We preprocess features following the guidelines in~\cite{10.1145/3643991.3644920} (e.g., normalization). 

\noindent\textbf{Selected models.}
We train three commonly used classifiers as in ~\cite{10.1145/3643991.3644920} for prediction of commit-level energy regression: Logistic Regression~\cite{lavalley2008logistic}, Random Forest~\cite{pal2005random}, and eXtreme Gradient Boosting~\cite{chen2015xgboost}. These models cover both linear and non-linear models and have been widely used as strong baselines in defect and regression prediction studies~\cite{10.1145/3643991.3644920,9197704,10.1145/3377811.3380351}.

\noindent\textbf{Data split and class imbalance.}
We randomly split the dataset into 80\% training and 20\% testing (8:2 split). Because energy regressions are typically rare compared to non-regressions, the training data are imbalanced. Following prior evidence that class re-balancing can improve regression prediction~\cite{tantithamthavorn2018impact,10.1145/3643991.3644920}, we apply SMOTE on the training portion only to balance minority (\textsc{Reg}) and majority (\textsc{NotReg}) classes. We keep the overall training strategy aligned with~\cite{10.1145/3643991.3644920} to facilitate comparability with established commit-level regression prediction settings.

\subsubsection{LLM-based predictor} We also evaluate an LLM-based approach that predicts whether a refactoring commit induces an energy regression using a structured prompt. For each refactoring commit in \practicalbenchmark{}, we include the metric values from Table~\ref{tab:extracted_metrics} in the prompt and ask the model to output a binary decision (\textsc{Reg} vs.\ \textsc{NotReg}). We use \texttt{gpt-5-mini} as the underlying model.

\noindent\textbf{Ablation study.}
To assess the contribution of different metric families, we performed an ablation study by excluding one family at a time from the prompt (e.g., removing static code metrics) and comparing prediction quality across settings.

\noindent\textbf{Incorporating semantic information.}
For semantic metrics, instead of providing the numerical diff embedding vector (which is not naturally interpretable to the LLM), we directly provide the textual diff hunks for modified Java production files and explicitly indicate that they are the commit diffs. To control prompt length, we include diffs for at most 10 modified production files, truncate each diff hunk to at most 6{,}000 characters, and cap the overall prompt length at 60{,}000 characters.

\subsubsection{Evaluation metrics}
We evaluate predictions using precision, recall, and F1-score for each class; however, identifying regressions is the primary objective and the dataset is imbalanced.

Let TP denote the number of regression commits correctly predicted as regressions, FP the number of non-regression commits incorrectly predicted as regressions, and FN the number of regression commits predicted as non-regressions.
\emph{Precision} is defined as
\[
\mathrm{Precision} = \frac{TP}{TP+FP}
\]
which measures how often predicted regressions are true regressions.
\emph{Recall} is defined as
\[
\mathrm{Recall} = \frac{TP}{TP+FN}
\]
which measures how many true regressions are successfully identified.
\emph{F1-score} is the harmonic mean of precision and recall:
\[
\mathrm{F1} = \frac{2 \cdot \mathrm{Precision}\cdot \mathrm{Recall}}{\mathrm{Precision}+\mathrm{Recall}}
\]
We report these metrics on the held-out test set for metric-based models and on the corresponding evaluated set for the LLM-based predictor.



==> sections/methodology_old.tex <==
\section{Methodology}
\label{sec:methodology}



\subsection{Data Collection}

Overall, we constructed two types of datasets to measure the impact of refactoring on energy consumption. The collection procedures are as follows. \modifyhaibo{TODO: the introduction should be in more details.}

\subsubsection{\microbenchmark{}}

To support a systematic study covering a broad range of refactoring types, we aim to construct a dataset that includes as many refactoring types as possible. We start with Martin Fowler's refactoring catalog in the second edition~\cite{fowler2018refactoring}, whose online catalog provides a comprehensive list of refactoring types and illustrative example code~\cite{onlinerefactoringcatalog}. However, we cannot directly use the online examples for energy measurement. First, the online catalog examples are primarily written in JavaScript, whereas our study focuses on Java. Second, many examples are incomplete as standalone programs and lack accompanying test suites; without executable tests that exercise the refactored behavior, the examples are unsuitable for repeated execution and before and after refactoring energy comparison.

To address these limitations, we used the first edition of Fowler's refactoring book, which provides Java-based examples. For each refactoring type, we match by name between the second edition catalog and the first edition book and manually extract the corresponding Java example code. Although these extracted examples are generally compilable, we found that most of them still do not include adequate tests that exercise the refactored code paths, which is essential for our measurement protocol. In addition, some refactoring types appear only in the second edition, so no Java example is available in the first edition.

Previous work has shown that LLMs can be effective in generating unit tests and translating code between languages~\cite{chen2024chatunitest,yuan2024evaluating,yang2024exploring,macedo2025intertrans}. We therefore leverage LLM to make the catalog executable under a uniform test-driven measurement workflow. In our pipeline, we use an LLM (gpt-5-mini in our experiments) in two roles:

\begin{description}[leftmargin=0pt]

\item[Workloads generation for \microbenchmark{}.] For each Java example code extracted, we prompt the LLM to generate five tests designed to exercise the refactored (modified) part of the code. If the generated tests do not compile or fail unexpectedly, we re-prompt the LLM to repair/regenerate tests, up to a predefined maximum number of attempts (ten attempts). \modifyhaibo{TODO: During the workloads generation, you should consider the diversity of the workloads, for example, if the input is List, the size of the list could affect the energy consumption. Previous studies~\cite{10.1145/2884781.2884869,10.1145/3168825} have shown that the input size of workloads has an impact on energy consumption and performance, thus, to obtain reliable energy consumption data, we try to generate tests with diverse input size. Specifically, ...}


\modifyhaibo{This section need to rewrite.}

\item[Translation and workloads generation for JavaScript code.] For refactoring types that do not have Java examples in the 1st edition, we manually extract the JavaScript example from the online catalog. We then ask the LLM to translate the example into compilable Java code and generate five tests that exercise the modified portion. As above, we iteratively regenerate the output if compilation or test execution fails, up to ten attempts.

\end{description}

Following this process, we obtain a refactoring catalog consisting of 68 refactoring types, each paired with (1) a compilable Java example code and (2) a test suite that exercises the modified code.



\subsubsection{\practicalbenchmark{}}


The refactoring programs in \microbenchmark{} are intentionally small and controlled. Although this enables targeted measurements, it cannot capture the richer context of real-world refactoring, where developers often combine multiple refactoring, and the surrounding complex context can influence energy outcomes. To complement \microbenchmark{} with a dataset that reflects refactoring in practice, we construct a second dataset, \practicalbenchmark{}, from real-world GitHub repositories.

\begin{description}[leftmargin=0pt]

\item[Initial refactoring commits collection.]
We collect candidate refactoring commits from two sources.
First, we incorporate refactoring commits from existing datasets and empirical studies~\cite{9136878,liu2025automated,nyirongo2025empirical,wang2025towards}. 


% Second, we independently crawl refactoring-related commits from the GH Archive~\cite{gharchive}, targeting commits between January 2015 and December 2025 (11 full years, covering the most recent complete years at the time of collection).

% To approximate the intention of refactoring from the developer's perspective, we apply commit-message filtering. Specifically, we retain commits whose message contains general refactoring keywords (e.g., \texttt{refactor} and \texttt{refactoring}) or refactoring type keywords drawn from (1) Martin Fowler's refactoring catalog~\cite{onlinerefactoringcatalog} and (2) the supported refactoring types listed by RefactoringMiner~\cite{refactoringminerlink}. To reduce non-refactoring noise, we exclude commits whose messages contain anti-words associated with bug fixing or documentation (e.g., \texttt{fix}, \texttt{bug}, \texttt{patch}, \texttt{doc}). Finally, because our study focuses on Java refactoring, we keep only commits that modify at least one \texttt{.java} file. These steps yield an initial pool of approximately 30 million candidate commits.


\item[Precondition checking.]
We further filter the candidate commits through a precondition-checking pipeline to ensure that each retained commit can support controlled execution and energy measurement.

\textit{Commit pairing.} For each candidate commit, we retrieve its parent commit via the GitHub API and discard merge commits (i.e., commits with multiple parents), ensuring a clean one-to-one before/after comparison.

\textit{Building system;} We restrict our study to Maven-based Java projects and require that a repository contains a \texttt{pom.xml} file at its root. 

\textit{Compilability.} We check both the refactoring commit and its parent commit and require that both versions compile successfully.


\item[Purity checking.]

We use test execution outcomes as an oracle to approximate refactoring purity. Concretely, we require the refactoring commit and its parent to be \textit{test-equivalent}. This criterion relies on three additional preconditions: (1) \textit{No test modifications:} we exclude commits that modify test files, because changing the oracle would invalidate test results comparison. (2) \textit{Coverage of modified code:} we require that the project's tests execute the code modified by the commit. We use JaCoCo~\cite{jacocolink} to obtain line-level coverage and intersect it with the commit's changed lines (retrieved via the GitHub API). If none of the changes are covered, the energy impact would be unobservable under test workload. (3) \textit{Test-equivalence:} after enforcing (1) and (2), we require that both versions pass the same tests, and discard commits that fail tests in either version. \modifyhaibo{TODO: The refactoring purity checking might need further filtering and consider using RefactoringMiner ASTDiff, or use human labeling to make sure the purity like in some previous work.}



\end{description} 

After applying these collection and precondition-checking steps, we obtain the practical benchmark, a dataset of real-world refactoring commits whose before/after refactoring versions are compilable, whose changes are exercised by tests, and whose behavior is preserved with respect to the test oracle. We used practical benchmark to study the energy impact of refactoring under realistic development scenarios. 




\subsection{Energy Consumption Measurements}

% We use JoularJX~\cite{noureddine-ie-2022} to measure the energy consumption of the program by executing their test suites. JoularJX is a Java-based agent for software power monitoring at the source code level that supports all operating systems. Energy measurements, even when conducted on the same computer, can be influenced by various factors. We followed best practices~\cite{energymeasurementlink,maquoi2025energy} to account for this. First, we freeze the system's configurations and ensure that only our software runs so other background system processes operate uniformly across all experiments. All experiments are conducted on a dedicated Mac mini server with macOS, an Apple M4 Pro chip, and 24GB of memory. We also warm up the machine hardware by conducting a one minute preliminary test before the actual measurements to stabilize the temperature. As pointed out by ~\cite{danglot2024can}, executing a project's test suite provides an effective method to approximate the total energy consumption of the project. In our case, we run the test suite of the projects 30 times to account for randomness~\cite{energymeasurementlink}. To prevent temperature increases between executions leading to artificially elevated energy consumption, we implement a one-minute cooling down period between each test suite execution. Lastly, we maintain stable room temperature for the testing equipment to mitigate any environmental factors that might affect the energy measurements. We build an energy measurement pipeline script to automate cloning project repositories, checkout to refactoring commit and its parent commit, preparing the JoularJX agent, and measuring energy consumption by executing the JUnit test suite 30 times per project, including a warm-up phase and rest intervals between each execution. The resulting data are stored in a json file for further analysis. In order to make sure that the refactoring commit and its parent commit are executed under the same context, every time we measured the energy consumption of the refactoring commit and its parent commit as a pair, the sequence to measure is shuffled to mitigate the bias that could be induced by execution order.

We use JoularJX~\cite{noureddine-ie-2022} to measure the energy consumption of the program by executing their test suites. JoularJX is a Java-based agent for software power monitoring at the source code level that supports all operating systems. It is developed on the basis of RAPL for Linux and Powermetrics for macOS. During the energy consumption measurement, we follow the established measurement guidelines~\cite{energymeasurementlink,maquoi2025energy} and keep the execution environment as stable as possible. All experiments run on a dedicated Mac mini server (macOS, Apple M4 Pro, 24\,GB RAM). During measurements, we disable non-essential services and avoid running unrelated workloads so that background activity remains consistent across runs.

For each version of the project (the refactoring commit and its parent), we repeatedly execute the project's JUnit test suite and record energy consumption values reported by JoularJX together with the execution time of the test. For refactoring examples in \microbenchmark{}, we directly execute their corresponding tests multiple times (default is one million) and obtain the energy consumption value by JoularJX. Following prior guidance that test executions can serve as a practical proxy workload for energy studies~\cite{danglot2024can}, we run the full test suite 30 repeats per version to reduce the impact of runtime variability. To control thermal effects, we (i) perform a short warm-up run (one minute) before collecting measurements, and (ii) insert a one minute cool-down interval between consecutive test executions.

We implement an automated measurement pipeline that clones repositories, checks out the two versions of each commit pair, configures the JoularJX agent, and executes the test suite 30 times per version with the warm-up and rest intervals described above. The pipeline stores raw per-run energy and timing data in JSON for subsequent statistical analysis. To avoid systematic bias from execution order, we randomize the order in which the two versions (parent versus refactoring commit) are measured within each pair~\cite{energymeasurementlink}. \modifyhaibo{TODO: How to minimize sources of non-determinism in the JVM during the measurement should be specified.}


\subsection{Metric Extraction}



\begin{table*}
\centering
\caption{Overview of our extracted metrics for a refactoring commit.}
\label{tab:extracted_metrics}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{l|l|l} 
\hline
\textbf{Category}                    & \textbf{Metrics}             & \textbf{Description}                                                              \\ 
\hline\hline
\multirow{3}{*}{Static code metrics~\cite{9197704,10.1145/3643991.3644920,10.1145/3377811.3380351}} & CK metrics                   & CK code metrics obtained by~\textcolor[rgb]{0.122,0.137,0.157}{static analysis.}  \\
                                     & Complexity                   & Cyclomatic complexity and~cognitive complexity.                                   \\
                                     & Code performance metrics          & Code metrics related with code performance.                                       \\ 
\hline
\multirow{8}{*}{Code change metrics~\cite{hindle2015green,10.1145/3377811.3380351}} & Code churn                   & Sum of lines added and deleted.                                                    \\
                                     & Entropy                      & Distribution of modified code across files.                                       \\
                                     & Line added                   & Total sum of lines added in a commit.                                             \\
                                     & Line deleted                 & Total sum of lines deleted in a commit.                                           \\
                                     & Changed hunks                & Number of changed code hunks.                                                     \\
                                     & Changed dirs                 & Number of modified directories.                                                   \\
                                     & Changed files                & Number of modified files.                                                         \\
                                     & Changed subsystems           & Number of modified subsystems.                                                    \\ 
\hline
\multirow{2}{*}{Test metrics~\cite{10.1145/3485136,bree2021automated}}       & Line coverage        & Line coverage ratio for modified files and lines.                                                              \\
                                     & Tests execution time         & Tests execution time.                                                             \\ 
\hline
\multirow{3}{*}{Refactoring metrics~\cite{10.1145/3485136,10.1145/2652524.2652538,6976079}} & Refactoring types total & Total number of refactoring types.                                           \\
                                     & Distinct refactoring types   & Total number of distinct refactoring types.                                  \\
                                     & Applied refactoring          & Specific applied refactoring in a commit.                              \\ 
\hline
\multirow{1}{*}{Semantic metrics~\cite{10174199}}    & Diff embedding               & Diff embedding for a commit.\\
\hline
\end{tabular}
\end{adjustbox}
\end{table*}



\modifyhaibo{TODO: The motivation for why extract these kinds of metrics should be stated, for example, some kinds of metrics are strongly correlated with energy consumption change, we should use statistically method to calculate the correlations among the energy consumption change and metrics change first, then we can know which kinds of metrics should be used for the refactoring-induced energy regression prediction.}


\modifyhaibo{TODO: Add another type of metrics, they are the runtime profile of the program before and after refactoring, including the execution time, JVM heap size, GC count, memory usage, CPU usage, and etc. This kind of information is corresponding to RQ3 and might be helpful for predicting the refactoring-induced energy regression.}



As shown in Table~\ref{tab:extracted_metrics}, we extract five families of metrics for each refactoring commit to answer RQ3. Our selection is guided by a simple principle: energy regression induced by refactoring is rarely explained by a single factor. Instead, it can be influenced by (i) the structural characteristics of the resulting code, (ii) the magnitude and dispersion of code edits, (iii) how the change is exercised by the test workload (since our energy is measured by running tests), (iv) the refactoring operations themselves, and (v) the semantic content of the transformation. Previous work on commit-level regression prediction and performance-aware testing has shown that combining signals from multiple perspectives can improve risk identification compared to using any single metric family alone~\cite{10.1145/3643991.3644920,10.1145/3377811.3380351,9197704}.

\noindent\textbf{Static code metrics.}
Static metrics describe the structural properties of code that may shape runtime behavior and resource usage. They have been widely adopted in regression prediction because they provide stable, implementation-oriented signals that are available before execution. We therefore extract three groups of static metrics:
(1) \emph{CK metrics} capture class-level structure (e.g., coupling and cohesion). These metrics are frequently used as general indicators of architectural complexity; higher coupling or larger classes can lead to larger execution footprints and less predictable performance effects when refactoring occurs.
(2) \emph{Complexity metrics} (cyclomatic and cognitive complexity) approximate control-flow complexity and reasoning difficulty. High complexity can imply more branches, nested control flow, and potentially different execution paths; when refactoring modifies such code, the risk of changing runtime cost (and thus energy) increases.
(3) \emph{Performance-related static metrics}~\cite{10.1145/3643991.3644920} capture static constructs that are commonly associated with code performance sensitivity (e.g., heavy control flow and lock).

\noindent\textbf{Code change metrics.}
Change metrics quantify \emph{how much} a commit edits and \emph{how widely} those edits spread. They are standard in defect prediction and regression prediction because larger and more scattered changes are harder to review and test, which increases the chance of unintended non-functional effects~\cite{10.1145/3377811.3380351,9197704}. We include:
(1) \emph{Code churn} (added$+$deleted lines), and separately (2) \emph{lines added} and (3) \emph{lines deleted} to differentiate expansion from removal.
(4) \emph{Changed hunks} measure edit fragmentation; many small hunks can indicate cross-cutting edits.
(5) \emph{Entropy} captures how evenly the change is distributed across files; commits with higher entropy tend to touch many files in a more uniform way, which has been used as a proxy for change scattering and risk.
We also include spread metrics that summarize how many units of the project are affected: (6) \emph{changed files}, (7) \emph{changed directories}, and (8) \emph{changed subsystems}. These metrics help distinguish refactorings localized to a module from those that propagate changes across architectural boundaries, which can be more likely to impact runtime characteristics.

\noindent\textbf{Test metrics.}
In our setting, energy is measured by repeatedly running the project test suite; therefore, test-related signals are critical for interpreting and predicting energy differences. We extract:
(1) \emph{Test execution time}, derived from the repeated test runs collected during energy measurement. Runtime is a direct contributor to energy; therefore, it provides an essential baseline signal for energy regression~\cite{10.1145/2652524.2652538}.
(2) \emph{Line coverage} signals how much code is executed by the tests. Using JaCoCo~\cite{jacocolink}, we computed coverage over modified files and lines, including \emph{the modified line coverage ratio}. This is important because if the changed lines are not covered, then the test workload is unlikely to expose any energy impact of the refactoring; conversely, increased modified line coverage increases observability and makes measured energy differences more attributable to the commitment~\cite{10.1145/3377811.3380351,10.1145/2652524.2652538}.

\noindent\textbf{Refactoring metrics.}
Refactoring metrics explicitly model \emph{what refactorings were applied}, which is information not captured by generic churn or complexity metrics. This is important because different refactoring operations (e.g., rename vs.\ extract) may have different tendencies to affect runtime behavior even when they have similar diff sizes. We therefore include:
(1) \emph{Refactoring types total}, the total number of refactoring operations detected in the commit;
(2) \emph{Distinct refactoring types}, the number of unique refactoring categories; and
(3) \emph{Applied refactoring}, a representation of which refactoring types appear (e.g., as a multi-hot vector over refactoring types). These features allow the model to learn patterns, such as whether commits that combine multiple structural refactorings are more likely to induce energy regression.

\noindent\textbf{Semantic metrics.}
Count-based metrics can miss \emph{what the change does}. To capture the semantic content of the refactoring edits, we compute a commit-level \emph{diff embedding}. We split the commit diff into hunks, obtain an embedding for each hunk using the OpenAI \texttt{text-embedding-3-large} model, and aggregate them (by averaging) into a single fixed-length (default 1024) vector. This representation provides a compact summary of the transformation content beyond surface statistics, enabling the predictor to distinguish, for example, API replacement refactoring from simple structural reorganizations even when their churn is similar.


Overall, our metrics are selected to provide complementary information for commit-level refactoring-induced energy regression prediction: structural properties of code (i.e., static metrics), magnitude and dispersion of edits (i.e., change metrics), observability under the test workload (i.e., test metrics), applied refactoring types (i.e., refactoring metrics), and transformation semantics (i.e., diff embeddings). This multi-view design follows the broader insight from the regression-prediction literature that combining heterogeneous signals is often necessary to identify regression events reliably~\cite{10.1145/3643991.3644920,10.1145/3377811.3380351,9197704}.



==> sections/results_old.tex <==
\section{Results}
\label{sec:result}

\subsection{RQ1: What is the impact of refactoring on energy consumption?}
\label{subsec:result_rq1}









To answer \rqone{}, we analyze the paired energy measurements collected for both \microbenchmark{} (catalog-style refactoring examples with generated tests) and \practicalbenchmark{} (real-world GitHub refactoring commits). \todo{in this sentence, you first mentioned micro-benchmark then practical benchmark but in subsequent paragraphs, you first discussed practical benchmark then micro. In RQ2, you also start discussing micro benchmark then practical benchmark. Usually, the readers expect the same order to be consistently used.} 

We use the paired statistical procedure described in Section~\ref{subsec:experiment_rq1_rq2} to determine whether the energy difference between the refactored version and its original version is statistically significant, and we report both significance and the direction of change (increase vs.\ decrease).

\paragraph{RQ1 results on \practicalbenchmark{}.}

\begin{table}[!htbp]
\centering
\caption{Information for the refactoring commits in \practicalbenchmark{}.}
\label{tab:practical_benchmark_information}
\begin{adjustbox}{width=0.7\linewidth}
\begin{tabular}{c|r} 
\hline
\textbf{Type}                                                                                                                                        & \textbf{Value}  \\ 
\hline\hline
\# of refactoring commits                                                                                                                                        & 479             \\
\# of projects                                                                                                                                       & 427             \\
Mean \# of refactoring types across all commits                                                                                                      & 10              \\
Median \# of refactoring types across all commits                                                                                                    & 3               \\
\# of energy consumption statistically significant different commits                                                                                 & 32              \\
\begin{tabular}[c]{@{}c@{}}\# of energy consumption statistically significant different commits \\whose energy consumption is increased\end{tabular} & 14              \\
\begin{tabular}[c]{@{}c@{}}\# of energy consumption statistic significant different commits \\whose energy consumption is decreased\end{tabular}     & 18              \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

Table~\ref{tab:practical_benchmark_information} summarizes the scale of \practicalbenchmark{} and the number of commits for which we observe statistically significant energy differences. The dataset contains 478 refactoring commits from 427 projects, and commits often include multiple refactoring types (mean 10 refactoring types per commit; median 3). This confirms that, in practice, refactoring is frequently performed as a bundle of operations rather than as a single isolated transformation.



\begin{figure}
    \centering
    \vspace{-3pt}    
    \includegraphics[width=0.7\linewidth]{resources/distribution_of_refactoring_commits.png}
    \vspace{-3pt}
     \caption{Distribution of energy consumption increased, unchanged, and decreased refactoring commits in \practicalbenchmark{}.}
     \Description{}
    \label{distribution_of_refactoring_commits}
\end{figure}



Out of 479 commits, only 32 commits (about 6.7\%) exhibit a statistically significant energy difference between the refactoring commit and its parent. Among these significant cases, 14 commits show increased energy consumption, and 18 commits show decreased energy consumption. \todo{the finding about most of the real world refactoring does not cause energy difference could be quite interesting but one problem is that we need to ensure that our measurement is valid because we only consider local energy consumption (e.g., energy consumption in remote server is not considered). it will be better to do a few sampling of the commits with no energy different and significant energy different to ensure that our measurement is valid (e.g., check whether the commit calls any server/third-party library that may incur additional non-local energy usage)} Figure~\ref{distribution_of_refactoring_commits} visualizes this distribution and highlights that the dominant outcome is not detectable change under the test workload: most commits fall into the unchanged group, while increases and decreases each account for only a small fraction of the dataset. Taken together, these results suggest that energy regressions induced by refactoring do occur in real projects, but they are relatively rare under test-suite workloads and measurement noise; at the same time, when energy does change significantly, the direction is not one-sided (refactoring can lead to either higher or lower energy usage). An implication for developers and researchers is that assumptions such as ``refactoring is energy-neutral'' or ``refactoring always hurts energy'' are not supported; instead, energy validation should be applied selectively, for example, when refactoring touches performance-sensitive code or when multiple structural refactorings are combined in a single commit. \modifyhaibo{It would be better to add an illustrative example to support this statement.}

\paragraph{RQ1 results on \microbenchmark{}.}




\begin{figure}
    \centering
    \vspace{-3pt}    
    \includegraphics[width=0.7\textwidth]{resources/rq1_group_level_energy_change.png}
    \vspace{-3pt}
     \caption{Group-level energy changes for the refactoring types whose energy consumption are statistically significant different in \microbenchmark{}.}
     \Description{}
    \label{rq1_group_level_energy_change}
\end{figure}




While \practicalbenchmark{} reflects real-world development, \microbenchmark{} provides a controlled setting where we can directly attribute energy differences to refactoring transformations and observe their behavior under repeated executions. Figure~\ref{rq1_group_level_energy_change} reports, for each type of refactoring whose before/after energy difference is statistically significant, how many paired measurement groups indicate an energy decrease, increase, or no change. A notable observation is that even within the same refactoring type, different instances can exhibit different directions between groups, and this finding is consistent with previous studies~\cite{10.1145/2652524.2652538}.\modifyhaibo{Add a table to show the statistic information of the micro-benchmark.}



\begin{figure}
    \centering
    \vspace{-3pt}    
    \includegraphics[width=0.8\linewidth]{resources/rq1_energy_change_ratio.png}
    \vspace{-3pt}
     \caption{Energy consumption change ratio for the refactoring types whose energy consumption are statistically significant different in \microbenchmark{}.}
     \Description{}
    \label{rq1_energy_change_ratio}
\end{figure}



Figure~\ref{rq1_energy_change_ratio} further quantifies the magnitude of energy change using the relative change ratio (after minus before, normalized by before) for each statistically significant refactoring type in \microbenchmark{}. The distributions show that some refactoring types tend to shift energy downward (negative median ratios), while others tend to shift energy upward (positive median ratios), and the spread can be large with visible outliers. For example, transformation patterns that change control flow (e.g., change reference to value) can yield noticeable reductions in energy in our examples, whereas other transformations (e.g., replacing error-code handling with exceptions) can yield substantial increases. The key takeaway is that even when refactoring is behavior-preserving, it can alter execution characteristics enough to produce large energy deltas in a controlled setting.

\paragraph{Energy change is strongly associated with execution-time change in \microbenchmark{}.}



\begin{figure}
    \centering
    \vspace{-3pt}    
    \includegraphics[width=0.48\textwidth]{resources/rq1_pearson.png}
    \vspace{-3pt}
     \caption{Pearson correlation heatmap for the energy consumption and other metrics in \microbenchmark{}.}
     \Description{}
    \label{rq1_pearson}
\end{figure}



To understand whether energy changes align with timing changes, Figure~\ref{rq1_pearson} \todo{the figure has been commented out but this sentence still refer to it?} shows a Pearson correlation heatmap computed on deltas (after minus before) for energy, time, and several lightweight code metrics in \microbenchmark{} as introduced in Section~\ref{subsec:experiment_rq1_rq2}. The strongest relationship is between energy delta and time delta (Pearson r = 0.70), indicating that, in our controlled examples, a major portion of energy variation is explained by execution time variation. In contrast, the change in the number of changed lines has near-zero correlation with energy delta, and complexity-related deltas show only weak association with energy delta. This suggests that simple size-based or complexity-only signals are insufficient to explain energy effects, even in small programs, while time remains an important mediator. A practical implication is that energy-aware validation should track execution time together with energy; reporting one without the other can make diagnosis difficult.

\paragraph{JIT effects: absolute energy changes, but relative refactoring impact is often stable.}

\begin{table}
\centering
\caption{JIT versus energy consumption correlation analysis for \microbenchmark{}.}
\label{tab:jit_correlation}
\begin{adjustbox}{width=0.6\linewidth}
\begin{tabular}{c|c|c} 
\hline
\textbf{Type}                   & \textbf{Pearson r} & \textbf{P-value}  \\ 
\hline\hline
Before refactoring              & -0.4328            & 7.456e-08         \\
After refactoring               & -0.4432            & 3.311e-08         \\
Refactoring energy change ratio & -0.0121            & 0.886             \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}



Because \microbenchmark{} programs are executed many times, the JVM JIT compilation can influence energy measurements. Table~\ref{tab:jit_correlation} reports the correlation analysis between the JIT settings and the energy values for the before and after versions, as well as for the energy change ratio. We observe a moderate correlation between JIT settings and absolute energy measurements for both the before and after versions (statistically significant p-values), but essentially no correlation between JIT settings and the energy change ratio (r close to 0, non-significant p-value). This indicates that JIT can shift the absolute energy baseline, but it does not systematically explain the relative before/after change ratio across refactorings in our dataset.



\begin{table}
\centering
\caption{Top five refactorings most influenced by JIT (difference in energy consumption change ratio, percentage points, JIT off - on).}
\label{tab:top_jit_impact_refactoring}
\begin{adjustbox}{width=0.6\linewidth}
\begin{tabular}{c|c} 
\hline
\textbf{Refactoring}                & \textbf{ratio delta}  \\ 
\hline\hline
Replace Loop with Pipeline          & 57.4140               \\
Replace Error Code with Exception   & -47.0877              \\
Replace Exception with Precondition & 34.7457               \\
Push Down Field                     & -34.0014              \\
Remove Parameter                    & -31.3927              \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}


However, JIT sensitivity is not uniform across refactoring types. Table~\ref{tab:top_jit_impact_refactoring} reporting the top five refactorings most influenced by JIT shows that for some types of refactoring (e.g., Replace Loop with Pipeline, Replace Error Code with Exception), the estimated change ratio can differ substantially between JIT-on and JIT-off executions. The implication is twofold: (i) refactoring-energy studies should keep JVM execution mode consistent within comparisons, and (ii) reporting JIT sensitivity (or at least acknowledging it) is important, especially for refactorings that modify hot code paths.


\noindent\textbf{Summary for RQ1.}
\todo{the current finding is a bit weak. please refer to some of the suggested findings by ChatGPT https://chatgpt.com/share/6a10c557-9ca4-83ea-a439-21730f5e554d and Gemini https://gemini.google.com/share/8e1de22751a3. For example, "Most real-world refactoring commits are effectively energy-neutral under test-suite workloads." will be a better finding} Across real-world refactoring commits, statistically significant energy changes are uncommon under test workloads, but they do occur and can be either increases or decreases. In controlled microbenchmarks, refactorings can produce substantial energy shifts and the direction depends on the refactoring type and context; energy deltas are strongly tied to execution-time deltas, and JIT can affect absolute energy while some refactorings remain sensitive in effect size.





\subsection{RQ2: Which refactoring types are more likely to influence energy consumption?}
\label{subsec:result_rq2}

We first answer RQ2 on \microbenchmark{}, where each refactoring type is evaluated in a controlled setting, and the before/after programs differ only by the intended refactoring. Figures~\ref{rq1_group_level_energy_change} and~\ref{rq1_energy_change_ratio} summarize the types of refactoring whose energy consumption differs significantly between the original and refactored versions. Figure~\ref{rq1_group_level_energy_change} reports, for each type of refactoring, the number of paired measurement groups that indicate a \emph{decrease}, \emph{increase} or \emph{no change} in energy. This view highlights the \emph{directional tendency} of each refactoring type in repeated measurements. Several refactoring types show a clear skew toward decreases or increases, while others exhibit mixed directions, suggesting that even in a controlled setup the energy impact is not uniform across instances. A practical implication is that the refactoring type alone can serve as a coarse risk indicator (some types are more likely to increase/decrease energy), but it cannot be reliably used to predict the energy usage for all scenarios (this inspires us to extract more metrics to predict energy regression in RQ3). %but it is not sufficient to deterministically predict the direction for every case (this inspires us to extract more metrics to predict energy regression in RQ3).

Figure~\ref{rq1_energy_change_ratio} complements this by quantifying the \emph{magnitude} of energy impact using relative change ratios (after minus before, normalized by before). The boxplots show that refactoring types differ not only in median effect but also in variability: some types have consistently small shifts, whereas others display wide spreads and outliers, indicating that the same refactoring type can yield very different energy outcomes depending on local code structure and executed paths. Importantly, for some refactoring types, the median ratio is clearly positive or negative, suggesting systematic energy tendencies in our examples.

Taken together, these two figures answer RQ2 for \microbenchmark{}: refactoring types differ in both (i) how often they lead to increases vs.\ decreases across repeated measurements (directional tendency) and (ii) how large those changes can be (magnitude and variance). The implication is that energy-aware refactoring validation can prioritize refactoring types that exhibit larger or more volatile energy change ratios in controlled examples, especially when they modify performance-sensitive structures (e.g., iteration style).


\begin{table*}
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{p{5.0cm}rrrrrrr}
\hline
\textbf{Pattern $S$} & \textbf{sup} & \textbf{base} & \textbf{conf} & \textbf{lift} & \textbf{OR} & \textbf{$\phi$} & \textbf{$p$ / $q$} \\
\hline\hline
\multicolumn{8}{l}{\textbf{Top 5 associated PAIRS for outcome: significant \& energy increase}} \\
$\{$Change Attribute Type, Rename Method$\}$ &
20 & 2.93\% & 15.00\% & 5.121 & 7.171 & 0.150 & 0.0170 / 0.5164 \\
$\{$Change Attribute Type, Extract Variable$\}$ &
10 & 2.93\% & 20.00\% & 6.829 & 9.500 & 0.148 & 0.0314 / 0.5164 \\
$\{$Extract Variable, Rename Attribute$\}$ &
11 & 2.93\% & 18.18\% & 6.208 & 8.426 & 0.139 & 0.0377 / 0.5164 \\
$\{$Change Attribute Type, Change Return Type$\}$ &
23 & 2.93\% & 13.04\% & 4.453 & 6.055 & 0.135 & 0.0251 / 0.5164 \\
$\{$Extract Variable, Rename Method$\}$ &
12 & 2.93\% & 16.67\% & 5.690 & 7.567 & 0.131 & 0.0445 / 0.5164 \\
\hline
\multicolumn{8}{l}{\textbf{Top 5 associated TRIPLES for outcome: significant \& energy increase}} \\
$\{$Change Attribute Type, Change Return Type, Rename Method$\}$ &
15 & 2.93\% & 20.00\% & 6.829 & 10.273 & 0.182 & 0.00742 / 0.2023 \\
$\{$Add Parameter, Change Attribute Type, Rename Parameter$\}$ &
10 & 2.93\% & 20.00\% & 6.829 & 9.500 & 0.148 & 0.0314 / 0.2023 \\
$\{$Add Parameter, Change Attribute Type, Rename Variable$\}$ &
10 & 2.93\% & 20.00\% & 6.829 & 9.500 & 0.148 & 0.0314 / 0.2023 \\
$\{$Add Parameter, Change Return Type, Extract Variable$\}$ &
10 & 2.93\% & 20.00\% & 6.829 & 9.500 & 0.148 & 0.0314 / 0.2023 \\
$\{$Add Parameter, Change Return Type, Rename Attribute$\}$ &
10 & 2.93\% & 20.00\% & 6.829 & 9.500 & 0.148 & 0.0314 / 0.2023 \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Association study for refactoring co-occurrence patterns and the outcome \emph{statistically significant \& energy increase} (minimum support $\ge 10$). 
\textbf{sup}: number of commits containing $S$; \textbf{base}: outcome base rate; \textbf{conf}: $P(Y{=}1\mid S)$; \textbf{lift}: conf/base; \textbf{OR}: odds ratio; $\boldsymbol{\phi}$: phi coefficient; $p$: Fisher exact test (two-sided); $q$: BH-FDR adjusted $p$ over all tested patterns (per $k$ and outcome).}
\label{tab:assoc_inc}
\end{table*}





\begin{table*}
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{width=0.88\textwidth}
\begin{tabular}{p{5.0cm}rrrrrrr}
\hline
\textbf{Pattern $S$} & \textbf{sup} & \textbf{base} & \textbf{conf} & \textbf{lift} & \textbf{OR} & \textbf{$\phi$} & \textbf{$p$ / $q$} \\
\hline\hline
\multicolumn{8}{l}{\textbf{Top 5 associated PAIRS for outcome: significant \& energy decrease}} \\
$\{$Change Variable Type, Move Attribute$\}$ &
10 & 3.77\% & 30.00\% & 7.967 & 12.943 & 0.201 & 0.00458 / 0.2065 \\
$\{$Change Parameter Type, Inline Variable$\}$ &
11 & 3.77\% & 27.27\% & 7.242 & 11.300 & 0.190 & 0.00615 / 0.2065 \\
$\{$Change Parameter Type, Remove Method Annotation$\}$ &
11 & 3.77\% & 27.27\% & 7.242 & 11.300 & 0.190 & 0.00615 / 0.2065 \\
$\{$Inline Variable, Move Method$\}$ &
11 & 3.77\% & 27.27\% & 7.242 & 11.300 & 0.190 & 0.00615 / 0.2065 \\
$\{$Extract And Move Method, Rename Parameter$\}$ &
20 & 3.77\% & 20.00\% & 5.311 & 7.929 & 0.178 & 0.00470 / 0.2065 \\
\hline
\multicolumn{8}{l}{\textbf{Top 5 associated TRIPLES for outcome: significant \& energy decrease}} \\
$\{$Change Method Access Modifier, Change Parameter Type, Change Variable Type$\}$ &
11 & 3.77\% & 27.27\% & 7.242 & 11.300 & 0.190 & 0.00615 / 0.9831 \\
$\{$Change Parameter Type, Change Return Type, Move Method$\}$ &
10 & 3.77\% & 20.00\% & 5.311 & 7.062 & 0.125 & 0.0504 / 0.9831 \\
$\{$Change Return Type, Inline Variable, Rename Variable$\}$ &
11 & 3.77\% & 18.18\% & 4.828 & 6.264 & 0.116 & 0.0603 / 0.9831 \\
$\{$Change Variable Type, Inline Variable, Rename Variable$\}$ &
11 & 3.77\% & 18.18\% & 4.828 & 6.264 & 0.116 & 0.0603 / 0.9831 \\
$\{$Change Variable Type, Move Method, Rename Variable$\}$ &
11 & 3.77\% & 18.18\% & 4.828 & 6.264 & 0.116 & 0.0603 / 0.9831 \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Association study for refactoring co-occurrence patterns and the outcome \emph{statistically significant \& energy decrease} (minimum support $\ge 10$). 
Column meanings are identical to Table~\ref{tab:assoc_inc}.}
\label{tab:assoc_dec}
\end{table*}


\todo{the first sentence in this section mentioned "We first answer RQ2 on Micro-benchmark," so there should be a "secondly,.." or "we then discuss". It is also unclear which paragraph presents the discussion for the practical benchmark. Is Table 5 and 6 about practical benchmarks? If yes, these should be noted in the table caption (Fig 2 and Fig 3 mentioned Micro-benchmark but other tables/fig did not mention practical benchmarks). Maybe we need to rewrite this paragraph to explain that unlike the microbenchmark where each program has one corresponding refactoring type, programs in the practical benchmark could have multiple refactoring types, and how you determine the refactoring types in the practical benchmark. also how many of the programs in the practical benchmarks has 1 refactoring type, how many has more than one or a table showing the statistics of the number of refactoring types exist in the practical benchmark will help readers to understand the characteristics of the benchmark}


Tables~\ref{tab:assoc_inc} and~\ref{tab:assoc_dec} summarize the top 5 refactoring co-occurrence patterns (pairs and triples) that are most strongly associated with statistically significant energy changes. Each row corresponds to a refactoring pattern $S$ and reports its \emph{support} (the number of commits containing $S$), the \emph{base rate} of the outcome in the full set of RefactoringMiner-success commits, and the \emph{confidence} $P(Y{=}1\mid S)$, i.e., the fraction of commits containing $S$ that also exhibit the target outcome. Lift further normalizes confidence by the base rate; lift values greater than $1$ indicate that commits containing $S$ are enriched for the outcome compared to an average commit. We also report odds ratio (OR) and $\phi$ as effect sizes, along with Fisher exact test $p$-values and BH-FDR corrected $q$-values that account for multiple hypothesis testing across many candidate patterns.


Across the significant \& energy-increase outcome (Table~\ref{tab:assoc_inc}), the top pairs and triples frequently involve type- and signature-related changes (e.g., \texttt{Change Attribute Type}, \texttt{Change Return Type}) together with variable extraction (e.g.,\texttt{Extract Variable}). These patterns show elevated confidence (e.g., 15--20\%) relative to the low base rate (2.93\%), yielding lift values typically above $4{\times}$ and up to about $6.8{\times}$. For the significant \& energy-decrease outcome (Table~\ref{tab:assoc_dec}), the top pairs are dominated by refactorings that adjust variable/parameter types, annotations, inlining, and method movement (e.g., \texttt{Change Variable Type}, \texttt{Inline Variable}, \texttt{Move Method}), with confidence around 20--30\% versus a base rate of 3.77\% (lift $\approx 5.3{\times}$ to $8.0{\times}$). These results suggest that energy-impactful refactorings can also manifest themselves as \emph{bundles} of related transformations that co-occur in the same commit.


Although several patterns achieve small unadjusted Fisher $p$-values, their BH-FDR $q$-values remain relatively large in this dataset, largely due to the small number of positive outcomes (14 significant increases and 18 significant decreases) and the large number of candidate patterns tested. Therefore, we interpret these co-occurrence results primarily as \emph{promising signals} rather than definitive causal factors. In practice, such patterns can be used as hypotheses to guide deeper investigations (e.g., controlling for commit size and number of refactoring operations, or validating on larger datasets) and as features for predictive models that aim to identify refactoring-induced energy regressions.


\noindent\textbf{Summary for \rqtwo{}.}
Across \microbenchmark{}, we observe clear heterogeneity across refactoring types: some types show a consistent directional tendency (mostly increases or mostly decreases) and some exhibit large and volatile energy-change ratios, indicating that refactoring type is a meaningful but coarse indicator of energy impact. In \practicalbenchmark{}, energy-impactful cases are rare, but the association analysis suggests that such cases often involve \emph{bundles} of co-occurring refactorings rather than isolated operations, with several enriched patterns combining related transformations (e.g., type/signature changes with extraction or inlining/movement). Overall, RQ2 indicates that energy influence is not uniformly distributed across refactoring types; instead, it concentrates in specific refactoring categories and co-occurrence patterns, motivating both targeted energy validation for higher-risk refactoring and richer, multi-factor analysis in \rqthree{}.


\subsection{RQ3: Why can refactoring result in energy consumption differences?}
\label{subsec:result_rq3}

The experiment result of \rqthree{}.


\subsection{RQ4: How effective are existing techniques in identifying refactoring-induced energy regressions?}
\label{subsec:result_rq4}


\begin{table*}
\centering
\caption{Experiment result of LLM-based classifier.}
\label{tab:llm_classifier_result}
\begin{adjustbox}{width=0.8\textwidth}
\begin{tabular}{c|ccccc|cc|cc|cc|c|c|c} 
\hline
\multirow{3}{*}{\textbf{Model }} & \multicolumn{5}{c|}{\textbf{Metrics }}                                                                                                                   & \multicolumn{6}{c|}{\textbf{Per class}}                                                                                                                                              & \multicolumn{3}{c}{\textbf{Macro avg }}                                                                   \\ 
\cline{2-15}
                                 & \multirow{2}{*}{\textbf{A }} & \multirow{2}{*}{\textbf{B }} & \multirow{2}{*}{\textbf{C }} & \multirow{2}{*}{\textbf{D }} & \multirow{2}{*}{\textbf{E }} & \multicolumn{2}{c|}{\textbf{Precision }} & \multicolumn{2}{c|}{\textbf{Recall }}             & \multicolumn{2}{c|}{\textbf{F1 }}                                                     & \multirow{2}{*}{\textbf{Precision }} & \multirow{2}{*}{\textbf{Recall }} & \multirow{2}{*}{\textbf{F1 }}  \\ 
\cline{7-12}
                                 &                              &                              &                              &                              &                              & \textbf{Reg} & \textbf{Not Reg}          & \textbf{\textbf{Reg}} & \textbf{\textbf{Not Reg}} & \textbf{\textbf{\textbf{\textbf{Reg}}}} & \textbf{\textbf{\textbf{\textbf{Not Reg}}}} &                                      &                                   &                                \\ 
\hline\hline
gpt-5-mini                       & Y                            & Y                            & Y                            & Y                            & Y                            & 0.0556       & 0.9787                    & 0.3571                & 0.7914                    & 0.0962                                  & 0.8751                                      & 0.5171                               & 0.5743                            & 0.4857                         \\
gpt-5-mini                       & N                            & Y                            & Y                            & Y                            & Y                            & 0.0396       & 0.9754                    & 0.2857                & 0.7677                    & 0.0696                                  & 0.8592                                      & 0.5075                               & 0.5267                            & 0.4644                         \\
gpt-5-mini                       & Y                            & N                            & Y                            & Y                            & Y                            & 0.0312       & 0.9728                    & 0.2143                & 0.7699                    & 0.0545                                  & 0.8595                                      & 0.5020                               & 0.4921                            & 0.4570                         \\
gpt-5-mini                       & Y                            & Y                            & N                            & Y                            & Y                            & 0.0110       & 0.9698                    & 0.0714                & 0.7591                    & 0.0190                                  & 0.8516                                      & 0.4904                               & 0.4153                            & 0.4353                         \\
gpt-5-mini                       & Y                            & Y                            & Y                            & N                            & Y                            & 0.0400       & 0.9775                    & 0.2857                & 0.7484                    & 0.0702                                  & 0.8477                                      & 0.5088                               & 0.5171                            & 0.4590                         \\
gpt-5-mini                       & Y                            & Y                            & Y                            & Y                            & N                            & 0.0238       & 0.9696                    & 0.1429                & 0.8230                    & 0.0408                                  & 0.8907                                      & 0.4967                               & 0.4833                            & 0.4658                         \\
\hline
\end{tabular}
\end{adjustbox}\par
\begin{tablenotes}
\footnotesize
\item{
\textbf{Y}: Current metrics are included; \textbf{N}: Current metrics are not included; \textbf{A}: Static code metrics; \textbf{B}: Code change metrics; \textbf{C}: Test metrics; \textbf{D}: Refactoring metrics; \textbf{E}: Diff embedding.
}
\end{tablenotes}
\end{table*}




\begin{table}
\centering
\caption{Experiment result of metrics-based classifier.}
\label{tab:metrics_classifier_result}
\begin{adjustbox}{width=0.6\linewidth}
\begin{tabular}{c|c|c|c|c} 
\hline
\textbf{ML Model }        & \textbf{Metrics} & \textbf{Precision } & \textbf{Recall } & \textbf{F1 }  \\ 
\hline\hline
Logistic Regression       & All              & 0.0311              & 0.2000           & 0.0533        \\
Random Forest             & All              & 0                   & 0                & 0             \\
eXtreme Gradient Boosting & All              & 0                   & 0                & 0             \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}


To answer \rqfour{}, we evaluate two families of approaches for predicting whether a refactoring commit induces an energy regression (\textsc{Reg}) or not (\textsc{Not Reg}) on \practicalbenchmark{}: (i) an LLM-based classifier prompted with the extracted information and (ii) metric-based machine learning classifiers trained on the same commit-level features. Because the dataset is highly imbalanced (only a small fraction of commits exhibit statistically significant energy increases), we report precision, recall, and F1 for the \textsc{Reg} class as the primary metrics, and we additionally report macro-averaged scores for the LLM to reflect balanced performance across both classes.

\paragraph{LLM-based classifier.}
Table~\ref{tab:llm_classifier_result} reports the performance of \texttt{gpt-5-mini} as a binary classifier under different prompt configurations. The left part of the table indicates which metric families are included in the prompt. The table then reports precision/recall/F1 for each class (\textsc{Reg} and \textsc{Not Reg}) and the macro-average across classes.

Two observations stand out. First, the LLM achieves consistently strong performance on the majority \textsc{Not Reg} class (precision around 0.97--0.98 and F1 around 0.85--0.89 across settings), but it struggles to precisely identify the minority \textsc{Reg} class. Even with all metric families included, the \textsc{Reg} precision is 0.0556 and the \textsc{Reg} F1 is 0.0962, indicating many false positives when the model predicts regression. This reflects the intrinsic difficulty of rare-event detection: when regressions are scarce, a model can obtain high overall accuracy by favoring the majority class, but precise identification of true regressions remains challenging.

Second, the ablation study shows that providing richer commit information generally helps. Using all metric families (A--E) yields the best macro-F1 (0.4857). Removing test metrics (C) causes the largest drop in macro-F1 (down to 0.4353), mainly because \textsc{Reg} recall collapses (0.3571 to 0.0714). This suggests that test-related signals, which summarize how the commit is exercised and how execution behaves under the test workload, are particularly informative for energy regression prediction. Removing semantic information (E) also reduces macro-F1 (to 0.4658) and substantially reduces \textsc{Reg} recall (to 0.1429), indicating that the change content itself (beyond numeric summary metrics) provides additional discriminative value. Overall, these results imply that LLM-based predictors benefit from multi-view evidence (A--E), but the remaining low \textsc{Reg} precision shows that the approach is not yet reliable as a standalone regression detector.

\paragraph{Metric-based classifiers.}
Table~\ref{tab:metrics_classifier_result} reports the performance of three standard metric-based models trained on all extracted metrics: Logistic Regression, Random Forest, and XGBoost. Logistic Regression achieves low precision (0.0311) and low recall (0.2000), resulting in an F1 of 0.0533 for the \textsc{Reg} class. Random Forest and XGBoost fail to identify any regression cases in the evaluated setting (precision/recall/F1 all 0), which indicates that these models cannot learn a stable decision boundary given the small number of positive outcomes and noisy labels.

\noindent\textbf{Summary for RQ4.}
Overall, both LLM-based and metric-based approaches find refactoring-induced energy regressions difficult to identify reliably, mainly due to the scarcity of regression cases and the resulting class imbalance. The LLM-based classifier benefits from combining multiple metric families, achieving the best macro-level performance when using all metrics (A--E), and the ablation results indicate that test metrics and semantic diff information contribute the most to regression recall. In contrast, the metrics-based classifiers perform poorly in our setting: logistic regression yields low precision and recall for the regression class, while random forest and XGBoost fail to detect any regression cases. These results suggest that existing commit-level predictors do not transfer well to refactoring-induced energy regression detection.
